Almost Optimal Streaming Algorithms for Coverage Problems

Maximum coverage and minimum set cover problems --collectively called coverage problems-- have been studied extensively in streaming models. However, previous research not only achieve sub-optimal approximation factors and space complexities, but also study a restricted set arrival model which makes an explicit or implicit assumption on oracle access to the sets, ignoring the complexity of reading and storing the whole set at once. In this paper, we address the above shortcomings, and present algorithms with improved approximation factor and improved space complexity, and prove that our results are almost tight. Moreover, unlike most of previous work, our results hold on a more general edge arrival model. More specifically, we present (almost) optimal approximation algorithms for maximum coverage and minimum set cover problems in the streaming model with an (almost) optimal space complexity of $\tilde{O}(n)$, i.e., the space is {\em independent of the size of the sets or the size of the ground set of elements}. These results not only improve over the best known algorithms for the set arrival model, but also are the first such algorithms for the more powerful {\em edge arrival} model. In order to achieve the above results, we introduce a new general sketching technique for coverage functions: This sketching scheme can be applied to convert an $\alpha$-approximation algorithm for a coverage problem to a $(1-\eps)\alpha$-approximation algorithm for the same problem in streaming, or RAM models. We show the significance of our sketching technique by ruling out the possibility of solving coverage problems via accessing (as a black box) a $(1 \pm \eps)$-approximate oracle (e.g., a sketch function) that estimates the coverage function on any subfamily of the sets.

==> RAM.tex <==
Here we consider the $k$-cover problem in the offline
setting. Specifically, here we require random access to the edge list
of vertices. Interestingly, we give a $(1-\frac 1 e
-\eps)$-approximation algorithm for $k$-cover in $\tilde{O}(n)$
time and a $\log\frac {1}{\eps}$-approximation algorithm for set
cover with outliers in $\tilde{O_{\lambda}}(n)$ time.

Badanidiyuru and Vondrak \cite{badanidiyuru2014fast} gives a
deterministic $1-\frac{1}{e}-\eps'$ approximation algorithm for monotone
submodular maximization with cardinality constraint, using $O(\frac n
{\eps'} \log\frac n {\eps'})$ queries to the submodular
function oracle. Remark that one query to a coverage function
may require $\Omega(m)$ time. \xxx{Done: what does this last sentence mean?}

\begin{algorithm*}%[!h]
  \textbf{Input:} A graph $G$ with sets \sets and elements \elements
  as well as $\eps'\in (0,1]$, and $k\in [1,n]$.
  \\
  \textbf{Output:} A $1-\frac 1 e -\eps'$ approximate solution to
  $k$-cover of $G$. 
	
  \begin{algorithmic}[1]
    \STATE Let $S=\emptyset$ and $d = \max_{a\in \sets}{\cov(a)}$.
    \STATE Let $w=d$
    \WHILE{$w\geq \frac{\eps'}{n}d$} 
    \FORALL{$a\in \sets$} 
    \IF{$|S\cup \set{a}|\leq k$ and $\cov(S\cup \set{a})-\cov(S)\geq w$}
    \STATE Add $a$ to $S$
    \ENDIF
    \ENDFOR
    \STATE Let $w = w(1-\eps') $
    \ENDWHILE
    \RETURN $S$.
  \end{algorithmic}
	
  \caption {Badanidiyuru and Vondrak~\cite{badanidiyuru2014fast} algorithm for $k$-cover}
  \label{Alg:offline:submo}
\end{algorithm*}



\begin{theorem}
In the offline setting, given random access to the edge
  list of vertices, for any arbitrary $\eps\in (0,1]$, with
  probability $1-\frac 1 n$ there exists a $(1-\frac 1 e
  -\eps)$-approximation algorithm for $k$-cover, with running time
  $\tilde{O}(n)$. 
\end{theorem}

%% \eps and \varepsilon

\begin{proof}
  Algorithm~\ref{Alg:offline:submo} is the interpretation of
  Badanidiyuru and Vondrak algorithm for $k$-cover problem. Note that,
  one can keep $\cov(S)$ and calculate $\cov(S\cup \set{a})-\cov(S)$
  by just checking the neighbors of $a$, in time linear in the degree
  of $a$. Thus, for an input graph $G$, the total running time of this
  algorithm is $\tilde{O}(|E|)$.

  Note that Theorem~\ref{thm:alg:kcover} bounds the number of edges of
  $H_{\leq n}$ used in Algorithm~\ref{Alg:main:SetCover} as
  $\tilde{O}(n)$. Therefore, Algorithm~\ref{Alg:offline:submo} on
  $H_{\leq n}$ has running time $\tilde{O}(n)$. We set
  $\eps'=\eps/2$. Algorithm~\ref{Alg:offline:submo} is a $1-\frac 1
  e -\eps'$ approximation algorithm. Thus, Using Algorithm~\ref{Alg:offline:submo}, Algorithm~\ref{Alg:main:KCover} is a
  $1-\frac 1 e -2\eps' = 1-\frac 1 e - {\eps} $ approximation
  algorithm. Now we show how to find $H_{\leq n}$ used in
  Algorithm~\ref{Alg:main:KCover} in $\tilde{O}(n)$ time.

  In order to find $H_{\leq n}$ we use a random process equivalent to
  the random process used in the definition of $H_{\leq n}$. We start
  with an empty graph $H$, and then iteratively pick an element
  uniformly at random without replacement. We assume that the $i$-th
  sampled element has the $i$-th minimum hash value among \elements.
  When we pick an element $b$ we add this vertex and
  $\min(\deg(b),\frac{n\log(1/\eps)}{\eps k})$ of its edges to
  the graph $H$ where $\deg(b)$ is the degree of $b$. We continue this
  process until the number of edges in $H$ is at least $\frac{24
    n\log(1/\eps)
    \log n{\log\log_{1-\eps}m)}\delta''}{(1-\eps)\eps^3}$.
  The final graph is by definition equivalent to $H_{\leq n}$. Remark
  that the number of edges in $H_{\leq}$ is $\tilde{O}(n)$. Thus, the
  total running time is $\tilde{O}(n)$. 
\end{proof}








==> prelims.tex <==
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%% NOT INCLUDED
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%

%% Problem definitions
We consider three \emph{coverage} problems in the paper. Everywhere we
have a ground set $\elements$ of elements and a family $\sets$ of sets
of elements.
%
In the \defterm{$k$-cover} problem, we look for $k$ sets in $\sets$
with the largest union size. When it is clear from the context, we may
use $\opt_k$ to denote the size of the union in this optimum solution.
%
The \defterm{set cover} problem, on the other hand, requires that all
elements in $\elements$ be covered while picking the minimum number of
sets from $\sets$.
%
We also define a third problem acting as a middle ground: in the
\defterm{set cover with outliers} problem, the goal is to find the
minimum number of sets covering at least a $1-\eps$ fraction of the
elements in $\elements$.

Our access to the input---i.e., the relationship between sets and
elements---is not unrestricted. In the \defterm{streaming} framework,
we focus on the so-called \defterm{edge arrival} model as opposed to
the more extensively studied \defterm{vertex arrival} model. In the
former, we get to know about the set-element relationships one at a
time, whereas in the latter, sets arrive and bring with them a list of
their elements.  (In this terminology, \emph{edges} represent the
relationship between sets \sets and elements \elements, and vertices
refer to the \sets.)  Moreover, the number of passes allowed for processing
the data may change the nature of the problem.

%In another setting, henceforth called the \defterm{RAM model}, we will
%have arbitrary access to the set-element relationship albeit at a
%price. More specifically, we may look at the list of elements in any
%set but each lookup (to read one element in any list) takes one unit
%of time.

We use this bipartite graph model of the input in
Section~\ref{sec:sketch} when talking about sketches and our
algorithms.  In that case, the graph is always bipartite and we refer
to its two parts by \emph{sets} \sets and \emph{elements} \elements.
In this model we use $\deg(v)$ for an element $v$ to denote the number
of sets covering it.

%% TODO
TODO: Talk very briefly about \defterm{MapReduce}.

Later on, we define the \defterm{$\eps$-noise oracle} which given a
subfamily of sets tells us an estimate of their union size within
$1\pm\eps$ precision.

%% Notations

For a graph $G$ and a subset $S$ of its vertices, we define $\Gamma(G,
S)$ to be the set of neighbors of $S$ in $G$.
%% Do we?
With some abuse of notation, the same is used to denote the size of
the neighborhood when this is clear from the context.

%%
\xxx{Mention all omitted proofs appear in the appendix.}


==> results.tex <==

In this paper we introduce a powerful sketch to summarize coverage functions. As the main property, we show that any $\alpha$-approximate solution to $k$-cover on this sketch is an $(\alpha -\epsilon)$-approximate solution to $k$-cover on the input, with high probability (see Theorem \ref{thm:str:main}). Interestingly, this sketch requires only $\tilde{O}(n)$ space.

In section \ref{sec:algorithms} using basic operations we design some algorithms for coverage problems based on our sketch. Indeed, in all of these algorithms we construct $\tilde{O}(1)$ independent instances of our sketch and use these sketches to solve the problems, without other direct access to the input. Simple definition of our sketch enables us to efficiently construct it in Streaming and Map-Reduce Settings and hence implement our algorithms in these settings. Interestingly, this provides almost tight algorithms for coverage problems in these settings. 
%
%
We present the following results for coverage problems in the streaming model.
\begin{theorem}In the streaming model, for any arbitrary $\epsilon\in (0,1]$, with probability $1-\frac 1 n$ we have
	\begin{itemize}
		\item \textbf{\ref{thm:str:kcover}:}
		A single pass $(1-\frac 1 e -\epsilon)$-approximation algorithm for $k$-cover, using $\tilde{O}(n)$ space.
		\item \textbf{\ref{thm:str:epscover}:}
		A single pass $(1+\epsilon)log(\frac 1 {\lambda})$-approximation algorithm for $(1-\lambda)$ cover , using $\tilde{O_{\lambda}}(n)$ space.
		\item \textbf{\ref{thm:str:setcover}:}
		A $p$ pass $(1+\epsilon)log(m)$-approximation algorithm for set cover, using $\tilde{O}(nm^{O(\frac{1}{p})}+m)$ space.		
	\end{itemize}
\end{theorem}

These are the first results presented for the edge arrival model. Indeed, these improve the approximation factor of all previously known results for the set arrival model~\cite{saha2009maximum,nisan2002communication,emek2014semi,chakrabarti2015incidence}, while the space may not be comparable (i.e. $\tilde{O}(n)$ versus $\tilde{O}(m)$).
Indeed, our result for streaming set cover gives an exponential improvement over Demaine et al.~\cite{demaine2014streaming} on both approximation factor and number of rounds, given the same space.

Next, we turn our attention to widely used distributed computation models like MapReduce.
\begin{theorem}In the distributed model, for any arbitrary $\epsilon\in (0,1]$, with probability $1-\frac 1 n$ we have
	\begin{itemize}
		\item \textbf{\ref{thm:mr:kcover}:}
		A three-round $(1-\frac 1 e -\epsilon)$-approximation algorithm for $k$-cover, where the loud on each machine is bounded by $\tilde{O}(|V|)$.
		\item \textbf{\ref{thm:mr:epscover}:}
		A three-round $(1+\epsilon)log(\frac 1 {\lambda})$-approximation algorithm for $(1-\lambda)$ cover, where the loud on each machine is bounded by $\tilde{O}_{\lambda}(|V|)$.
		\item \textbf{\ref{thm:mr:setcover}:}
		An $r$-round $(1+\epsilon)log(m)$-approximation algorithm for set cover, where the load on each machine is bounded by $\tilde{O}(nm^{O(\frac{1}{r})}+m)$.
	\end{itemize}
\end{theorem}

While size of the input graph may be as large as $\Omega(nm)$, we show that we can query only $\tilde{O}(n)$ bits of the input to construct our sketch. This enable us to design a $(1-\frac 1 e-\epsilon)$-approximation algorithm in the classical RAM model \cite{aho1974design} running in $\tilde{O}(n)$ time. Indeed, this is the fastest $(1-\frac 1 e -\epsilon)$-approximation algorithm in classical RAM model.

\begin{theorem}In the RAM model, for any arbitrary $\epsilon\in (0,1]$, with probability $1-\frac 1 n$ there exist a $(1-\frac 1 e -\epsilon)$-approximation algorithm for $k$-cover, with running time $\tilde{O}(n)$.
\end{theorem}

On the hardness side, we show that any $(0.5+\epsilon)$-approximation streaming algorithm for $k$-cover requires $\Omega(n)$ space. This holds even for streaming algorithm with several passes.
Interestingly, this hardness result holds for a very simple input in which $k=1$ and $m=2$. Therefore, there is no hope to find a $(0.5+\epsilon)$-approximation streaming algorithm for $k$-cover using $o(n)\Phi(m,k)$ space, where $\Phi(m,k)$ is any arbitrary function of $m$ and $k$ but independent of $n$.

\begin{theorem}\label{thm:str:hard}
	Any $(0.5+\epsilon)$-approximation multi-pass streaming algorithm for $k$ cover requires $\Omega(n)$ space in total. This holds even for $k=1$ and $m=2$.
\end{theorem}


Indeed, edge arrival version of the coverage problems
gives us more flexibility to use this approach for other problems. 
As an instance, in Appendix \ref{sec:DominatingSet}, using a simple reduction we give the first nontrivial streaming algorithm for the dominating set problem.  Specifically, we show a $p$ pass $log(n)$-approximation streaming algorithm for dominating set, using $\tilde{O}(n^{1+O(\frac{1}{p})})$ space, where $n$ is the number of vertices. 


The notion of our sketch is fairly relevant to the notion of $l_0$ sketches \cite{cormode2003comparing}. $l_0$ sketches are basically defined to estimate the value of coverage functions (see Appendix \ref{Apx:O(nk)} for a formal definition of $l_0$ sketch). Indeed, one may maintain $n$ $l_0$ sketches and perfectly estimate the value of the coverage function of a single feasible solution of size $k$, with high probability. However, as there are $n \choose k$ different choices for a solution of size $k$, there is a huge blow up on the probability of failure of one of these solutions. In Appendix \ref{Apx:O(nk)}, we show a straightforward analyze to approximate $k$ cover using $l_0$ sketches with $\tilde{O}(nk)$ space. Notice that, the space required by the algorithm that uses $l_0$ sketches is quite larger than our sketch.


==> table.tex <==
\begin{table*}
\begin{center}
	\begin{tabular}{ ||c|c|c|c|c|c|| } 
		\hline
		Problem  & Reference & No.Passes & Approximation & Space & Comment \\
		\hline
		\hline 
		$k$ cover & \cite{saha2009maximum} & $1$ & $ 1/ 4 $ & $\tilde{O}(m)$ & set arrival \\ 
		$k$ cover & Here & 1 & $1- 1/ e -\epsilon$ & $\tilde{O}(n)$ & edge arrival \\ 
		%
		\hline
		Set cover w outliers & \cite{emek2014semi, chakrabarti2015incidence} & $p$ & $O(min(n^{1/(p+1)},e^{-1/p}))$ & $\tilde{O}(m)$ & set arrival \\
		
		Set cover w outliers & Here & $1$ & $(1+\epsilon)\log( 1/ {\lambda})$ & $\tilde{O}_{\lambda}(n)$ & edge arrival \\
		%
		\hline
		Set cover & \cite{chakrabarti2015incidence,saha2009maximum} & $p$ & $(p+1)n^{1/(p+1)}$ & $\tilde{O}(m)$ & set arrival \\
		
		Set cover & \cite{demaine2014streaming} & $4^k$ & $4^k\log(n)$ & $\tilde{O}(nm^{1/k})$ & set arrival \\		
		Set cover & Here & $p$ & $(1+\epsilon)\log(n)$ & $\tilde{O}(nm^{O(1/p)}+m)$ & edge arrival \\
		%
			\hline
	\end{tabular}
\end{center}		
	\caption{Algorithms in the streaming setting}
\end{table*}

\begin{table*}
\begin{center}
	\begin{tabular}{ ||c|c|c|c|c|c|| } 		
		\hline
		Problem  & Reference & No. Rounds & Approximation & Load per Machine &  Comment \\ 
		\hline 
		\hline
		$k$ cover & \cite{KMVV13} & 			  $O(\frac{1}{\epsilon\delta}\log(m))$ & $1- 1/ e-\epsilon$ & $O(mkn^{\delta})$ & submodular functions \\ 
		$k$ cover & \cite{MZ15} & 			  $2$ & $0.54$ & $max(m k^2, mn/k)$ & submodular functions \\ 
		
		$k$ cover & Here & 			  $3$ & $1- 1/ e -\epsilon$ & $\tilde{O}(n+m)$ & - \\ 
		%
		\hline
		Set cover w outliers & Here & $3$ & $(1+\epsilon)\log( 1/ {\lambda})$ & $\tilde{O}(n+m)$ & - \\	
		%	
		\hline
		Set cover & Here & 			  $r$ & $(1+\epsilon)\log(n)$ & $\tilde{O}(nm^{O(1/r)}+m)$ & - \\
		%
		\hline	
	\end{tabular}
\end{center}
	\caption{Algorithms in the distributed settings}
\end{table*}	


\iffalse
\begin{table*}
\begin{center}
	\begin{tabular}{ ||c|c|c|c|c|| } 		
		\hline
		Problem  & Reference & Approximation & Running time & Comment \\ 
		\hline 
		\hline 
		 $k$ cover & \cite{badanidiyuru2014fast} & $1- 1/ e -\epsilon$ & $\tilde{O}(nm)$ & submodular functions  \\ 
		$k$ cover & Here & $1- 1 /e -\epsilon$ & $\tilde{O}(n)$ &  - \\ 
		\hline	
	\end{tabular}
\end{center}
	\caption{Algorithms in the RAM model}
\end{table*}
\fi


==> temp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Further Properties}


Lets construct $H^{full}_{\leq n}$ from $H_{\leq n}$ by connecting vertices of degree $\frac{log(1/\epsilon)n}{\epsilon k}$ in $B$ to all vertices in $A$.

\begin{lemma}
Let $k'$ be the size of the set cover on the input graph $G$, and let $k=log(\frac{1}{\lambda})k'$. $Greedy(k,H^{full}_{\leq n})$ covers $1-\lambda$ fraction of the vertices in $H^{full}_{\leq n}$. 
\end{lemma}
\begin{proof}
Set $p^*$ such that $H'_{p^*}=H_{\leq n}$. Remark that $H_{p^*}$ is an induced subgraph of $G$ that contains all vertices in $A$. Thus, a set cover in $G$ is a set cover in $H_{p^*}$ as well. Moreover, $H^{full}_{\leq n}$ is a supergraph of $H_{p^*}$. Thus, a set cover in $G$ is a set cover in $H^{full}_{\leq n}$ as well. This means that size of the minimum set cover in $H^{full}_{\leq n}$ is at most $k'$. By selecting $k=log(\frac{1}{\lambda})k'$ vertices based on $Greedy$ on such a graph we cover at least $1-\lambda$ of the vertices.
\end{proof}


\begin{lemma}
Let $k'$ be the size of the set cover on the input graph $G$, and let $k=log(\frac{1}{\lambda})k'$. $Greedy(k,H_{\leq n})$ covers $1-\lambda-O(log(\frac{1}{\lambda})\epsilon)$ fraction of the vertices in $G$, with probability $1-3e^{-\delta''}$. 
\end{lemma}
\begin{proof}
Using Lemma \ref{lm:loglambda} we know that there exists a solution of size $k'$ on $H_{\leq n}$ that covers at least $1-log(\frac{1}{\lambda})\epsilon$ fraction of the vertices of $H_{\leq n}$. Thus, $Greedy(k,H_{\leq n})$  covers at least $(1-\lambda)(1-log(\frac{1}{\lambda})\epsilon)\geq 1-\lambda-log(\frac{1}{\lambda})\epsilon$ fraction of the vertices of $H_{\leq n}$. This together with Lemma \ref{thm:str:main} says that $Greedy(k,H_{\leq n})$ covers at least $1-\lambda-log(\frac{1}{\lambda})\epsilon$ fraction of the vertices of $G$, with probability $1-3e^{-\delta''}$.
\end{proof}


\begin{lemma}\label{lm:H<n:1-2eps'}
Let $k^*$ be the size of the set cover on the input graph $G$. Let $\epsilon$ be an arbitrary small number and let $\lambda\in (0,\frac 1 e]$, and let $k'=(1-\epsilon)k^*$ and $k=log(\frac{1}{\lambda})k'$. $Greedy(k,H_{\leq n})$  covers at least $1-\lambda-2 log(\frac{1}{\lambda})\epsilon$ fraction of vertices in $H_{\leq n}$.
\end{lemma}
\begin{proof}
Using Lemma \ref{lm:loglambda} we know that there exists a solution of size $k^*$ on $H_{\leq n}$ that covers at least $1-(1-\epsilon)log(\frac{1}{\lambda})\epsilon \geq 1- log(\frac{1}{\lambda})\epsilon$ fraction of the vertices of $H_{\leq n}$. 

Remark that the marginal increase of $f(Greedy(i,G))$ is decreasing as $i$ increases, i.e. $f(Greedy(i+1,G))-f(Greedy(i,G))\leq f(Greedy(i,G))-f(Greedy(i-1,G))$. Therefore, we have $f(Greedy((1-\epsilon)log(\frac{1}{\lambda})k^*,G))\geq (1-\epsilon)f(Greedy(log(\frac{1}{\lambda})k^*,G))$.
Thus, $Greedy(k,H_{\leq n})$ covers at least
\begin{align*}
(1-\epsilon)(1-\lambda)(1-log(\frac{1}{\lambda})\epsilon)&\geq 1-\lambda-log(\frac{1}{\lambda})\epsilon-\epsilon\\
&\geq 1-\lambda-2 log(\frac{1}{\lambda})\epsilon
\end{align*}
fraction of the vertices of $H_{\leq n}$. 
\end{proof}
